End-to-End Real-time Catheter Segmentation with Optical Flow-Guided Warping during Endovascular Intervention

Accurate real-time catheter segmentation is an important pre-requisite for robot-assisted endovascular intervention. Most of the existing learning-based methods for catheter segmentation and tracking are only trained on small-scale datasets or synthetic data due to the difficulties of ground-truth annotation. Furthermore, the temporal continuity in intraoperative imaging sequences is not fully utilised. In this paper, we present FW-Net, an end-to-end and real-time deep learning framework for endovascular intervention. The proposed FW-Net has three modules: a segmentation network with encoder-decoder architecture, a flow network to extract optical flow information, and a novel flow-guided warping function to learn the frame-to-frame temporal continuity. We show that by effectively learning temporal continuity, the network can successfully segment and track the catheters in real-time sequences using only raw ground-truth for training. Detailed validation results confirm that our FW-Net outperforms state-of-the-art techniques while achieving real-time performance.

==> 1_intro_backup.tex <==
\section{INTRODUCTION} \label{Sec:Intro}
%As an alternative to open surgery, endovascular intervention offers many advantages, including quicker recovery period, less discomfort for patients, local or regional anesthesia instead of general anesthesia, smaller incisions, stability, and more importantly, fewer risks for patients who have other high-risk medical conditions~\cite{simaan2018medical}. Recently, with the joint efforts from multidisciplinary  fields, endovascular interventions have become an effective treatment approach for vascular diseases. Many relevant problems for endovascular interventions have been actively investigated, for example, robotic design~\cite{thakur2009design, abdelaziz2019toward, bian2013enhanced}, surgical perception feedback~\cite{zhao2019cnn}~\cite{dagnino2018haptic}, or learning-based endovascular navigation~\cite{chi2018learning}~\cite{chi2018trajectory}.

%Catheters and guidewires are extensively used in many cardiac procedures such as ablation, angioplasty, and valvuloplasty. Due to its wide range of applications, catheter segmentation in X-ray fluoroscopic images is a crucial task for several clinical problems such as surgical action prediction, 3D reconstruction, or collision prediction. However, 
As an alternative to open surgery, endovascular intervention offers many advantages, including quicker recovery period, less discomfort for patients, local or regional anesthesia instead of general anesthesia, smaller incisions, stability, and more importantly, fewer risks for patients who have other high-risk medical conditions~\cite{simaan2018medical}. Endovascular intervention involves the manipulation of catheters and guidewires to reach target areas in the vasculature to deliver a treatment (e.g. stenting, drug \cite{rafii-tari_current_2014}). Such tasks require a high level of technical skill to avoid damage to the vessel wall, which could result in perforation and hemorrhage, or dissection and organ failure, both of which can be fatal. Despite the advantages of its minimally invasive approach, endovascular procedure still presents some limitations such as limited sensory feedback, misalignment of visuo-motor axes, and the need for high dexterity \cite{benavente_molinero_haptic_nodate}. Robotics and computer assistance have been integrated into the clinical workflow to provide augmentation of surgical skills in terms of enhanced dexterity and precision (\cite{thakur2009design, abdelaziz2019toward, bian2013enhanced, zhao2019cnn, dagnino2018haptic, chi2018learning, zhu2017deep}).  


\begin{figure}[!t] 
    \centering
    % \includegraphics[width=0.99\linewidth, height=0.75\linewidth]{figures/1_intro/all_5.jpg}
    \includegraphics[width=0.99\linewidth, height=0.8\linewidth]{figures/1_intro/intro.pdf} 
    \vspace{0.2ex}
    \caption{Catheter and guidewire segmentation in 2D X-ray fluoroscopy sequences. \textbf{Top row:} The X-ray image. \textbf{Bottom row:} An illustration of segmented results of aortic phantom.}
    \label{Fig_intro} 
\end{figure}
Previous work from our group in the Hamlyn Centre focused on the development of a robotic platform – the CathBot – for endovascular intervention with the goal of improving dexterity and navigation, by providing robot assistance and haptic feedback to the surgeon.
The CathBot \cite{abdelaziz2019toward} comprises a versatile master-slave setup and navigation framework. Unlike previous platforms, the robot can be safely integrated and used in MR environments thanks to pneumatic actuation and additive fabrication. The master robot is an intuitive HMI which mimics the human motion pattern (i.e. grasping, push/pull or rotary motion) and provides haptic feedback to the users generated by the navigation systems as described below. Motions are mapped to an MR-safe slave robot which manipulates guidewires and catheters. 
The navigation system was described in depth in \cite{dagnino2018haptic, benavente_molinero_haptic_nodate} and comprises two core functions: 1) Intra-operative visualisation of the surgical imaging data to the operator and 2) generation of dynamic active constraints for haptic feedback rendered to the master based on visual information extracted from live imaging data. In brief, instruments (catheter, guidewire) were tracked in the imaging live stream for the angiography system for determination of tip positions. Simultaneously, the corresponding vessel wall was detected and tracked to obtain a distance metric. The latter is combined with current motor currents to update viscous friction models for both axes that are rendered to the operator through the master device. In detail, friction was decreased to a minimum if the tip of the instrument is located in the centre of the vessel. The modelled friction increases if the detected distance between instrument and wall decreases.
Such a vision-based force sensing through shape and position analysis of the tip of catheter and the vasculature is a promising solution as demonstrated in \cite{dagnino2018haptic,benavente_molinero_haptic_nodate}. However, in clinical applications, damages to the vessels are generated not only by the contact of the instrument tip with the vessel wall, but by the contacts between the entire instrument and the endothelial wall. Therefore, the tracking of the entire instrument is required such that the contact forces between the catheter and guidewire with the endothelial wall can be minimised. Furthermore, this information can be used to for task assessment of the surgical procedure as well \cite{Rafii-Tari2017}.

Building on our previous work, we propose a real-time catheter segmentation framework enabling the entire catheter tracking on x-ray fluoroscopy.

Autonomous catheter segmentation is not a trivial task for two main reasons. Firstly, in the X-ray image, catheters can be easily confused with other similar linear structures like blood vessels due to its low contrast. Secondly, during clinical trials, catheters and guidewires can  have a sudden and large deformation movement. This leads to the fact that traditional methods~\cite{brost2009_tracking, brost2010respiratory, yatziv2012_multiple, baert2003_guidewire_tracking} based on primitive features of catheter appearance have limited generality and would not be able to segment catheters and guidewires in real-time and dynamic surgical environments. 

Recently, machine learning, especially deep learning has been widely chosen as a novel approach for medical image segmentation~\cite{ronneberger2015_UNet, milletari2016_VNet, wang2018deepigeos}. The effectiveness of deep learning comes from the ability to handle a large amount of input data~\cite{lecun2015deep}. However, this advantage becomes a potential problem in catheter segmentation since it is not easy to create large-scale datasets with pixel-wise labels. This is because the annotation task requires a certain amount of medical expertise, while manually labeling is very tedious, especially for objects with elongated structures such as catheters and guidewires. Due to these challenges, recent deep learning methods for catheter segmentation mainly train on a very small dataset~\cite{breininger2018_multihead}~\cite{breininger2018intraoperative}, use synthetic data~\cite{yi2019_rnn_synthetic}, or create groundtruth based on a particular observation about pixel intensity~\cite{vlontzos2018deep}. These assumptions technically limit the power of deep learning and the generality of the methods.


In this paper, we propose Flow-guided Warping Net (FW-Net), a new end-to-end framework for catheter segmentation in 2D X-ray fluoroscopy sequences. Our hypothesis is that deep network can be trained using the raw groundtruth while the overall accuracy can be improved by effectively learning the temporal continuity from X-ray sequences. In particular, we first create the raw groundtruth using a vision-based approach~\cite{ma2018novel}, then we design FW-Net with three modules: i) a segmentation network, ii) a flow network, and iii) a novel flow-guided warping function. We train FW-Net on raw groundtruth data and employ the flow-guided warping function to learn the temporal continuity between consecutive X-ray frames. This will encourage the network to predict based on both the raw groundtruth and sequential information, hence potentially improve the overall accuracy.

The rest of the paper is organized as follows. We review the related work in Section~\ref{Sec_rw}, then describe our MRI safe robotic platform in Section~\ref{Sec_robot} for data collection. In Section~\ref{Sec_method}, we present the new end-to-end architecture for effectively segmenting the catheter from raw groundtruth. The experimental results are presented in Section~\ref{Sec_exp}. Finally, we conclude the paper and discussed the future work in Section~\ref{Sec_con}.



%%%\cite{Rafii-Tari2017}
